Learning Goal-Conditioned Policies Offline with Self-Supervised Reward Shaping

Developing agents that can execute multiple skills by learning from pre-collected datasets is an important problem in robotics, where online interaction with the environment is extremely time-consuming. Moreover, manually designing reward functions for every single desired skill is prohibitive. Prior works targeted these challenges by learning goal-conditioned policies from offline datasets without manually specified rewards, through hindsight relabelling. These methods suffer from the issue of sparsity of rewards, and fail at long-horizon tasks. In this work, we propose a novel self-supervised learning phase on the pre-collected dataset to understand the structure and the dynamics of the model, and shape a dense reward function for learning policies offline. We evaluate our method on three continuous control tasks, and show that our model significantly outperforms existing approaches, especially on tasks that involve long-term planning.

==> limitations.tex <==
\section{Limitations}

Our work presents a method that learns a goal-conditioned state-reaching policy without any supervised reward signal nor online interactions with the environment.
However, it relies on the availability of a pre-collected dataset of trajectories, whose coverage on the state space should be large enough for proper policy training.
Although such data can be already available, as for the RoboYoga Walker task, or that offline dataset collection could be done with random policies, as we did on the UMaze and Pusher tasks, this step can be challenging for other environments.
Moreover, we evaluated our method exclusively on simulated environments, and we did not perform any experiments on real robots, for which pre-collected dataset with expert demonstrations can be available~\citep{chebotar2021actionable}.

==> main.tex <==
\input{header}

\begin{document}

\input{main_core}

\end{document}
